An Improved Analysis of Langevin Algorithms with Prior Diffusion for Non-Log-Concave Sampling

Understanding the dimension dependency of computational complexity in high-dimensional sampling problem is a fundamental problem, both from a practical and theoretical perspective. Compared with samplers with unbiased stationary distribution, e.g., Metropolis-adjusted Langevin algorithm (MALA), biased samplers, e.g., Underdamped Langevin Dynamics (ULD), perform better in low-accuracy cases just because a lower dimension dependency in their complexities. Along this line, Freund et al. (2022) suggest that the modified Langevin algorithm with prior diffusion is able to converge dimension independently for strongly log-concave target distributions. Nonetheless, it remains open whether such property establishes for more general cases. In this paper, we investigate the prior diffusion technique for the target distributions satisfying log-Sobolev inequality (LSI), which covers a much broader class of distributions compared to the strongly log-concave ones. In particular, we prove that the modified Langevin algorithm can also obtain the dimension-independent convergence of KL divergence with different step size schedules. The core of our proof technique is a novel construction of an interpolating SDE, which significantly helps to conduct a more accurate characterization of the discrete updates of the overdamped Langevin dynamics. Our theoretical analysis demonstrates the benefits of prior diffusion for a broader class of target distributions and provides new insights into developing faster sampling algorithms.

==> 0_config/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\hanze}[1]{{\textcolor{orange}{#1} }}

\newcommand{\issue}[1]{{\textcolor{purple}{#1} }}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rvzeta{{\mathbf{\zeta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\cR{{\mathcal{R}}}
\def\EE{{\mathbb{E}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vrho{{\bm{\rho}}}
\def\vzeta{{\bm{\zeta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

%

\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny{#1}};}}
% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\newcommand{\der}{\mathrm{d}}
\newcommand{\fder}{\mathrm{D}}
\newcommand{\rgrad}{\mathrm{grad}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Table settings

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3\arrayrulewidth}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}


==> 0_contents/020preliminaries_backup.tex <==
\section{Problem Setup}
\label{sec:problem_setup}
This section will first introduce the notations commonly used in the following sections. 
Then, we will show the main algorithm, i.e., Langevin Algorithm with Prior Diffusion as Alg~\ref{alg:lapd}, and the slight differences between our version and that provided in~\citet{freund2022convergence}.
Besides, we will also explain the intuitions about designing Alg~\ref{alg:lapd}.
Due to the high dependency on the convexity of $f$ in such a design, we will introduce its effect on the convergence analysis, which also leads to the main difficulty when we expect to extend such a result to a broader class of target distributions with the second kind of proof shown in Section~\ref{sec:related_work}.



When the dataset is given as $\vz$, we consider sampling from a posterior distribution over parameter $\vw\in \R^d$:
\begin{equation*}
    p(\vw | \vz) \propto p(\vz | \vw)\pi(\vw) \propto \exp\left(-U(\vw)\right) \coloneqq p_*(\vw).
\end{equation*}
The potential $U\colon \R^d \rightarrow \R$ can be decomposed as $ U(\vw) = f(\vw) + g(\vw)$,
where $f,g\colon \R^d \rightarrow \R$.
This formulation is general in machine learning tasks. From a Bayesian view, we can divide the regularized empirical risk minimization loss to two parts: we can consider $f$ as the negative log-likelihood (loss function) and $g$ as the negative log-prior (regularization term).
Correspondingly, for any distribution $p$, we decompose KL divergence between $p$ and the target distribution $p_*$, as follows
\begin{equation}
    \label{eq:kl_compos_func}
    \mathrm{KL}\left(p\|p_*\right) = \underbrace{\mathbb{E}_{\rvw\sim p}\left[f(\rvw)\right]}_{\mathrm{Term\ 1}} + \underbrace{\mathbb{E}_{\rvw\sim p}\left[g(\rvw)+\log p(\rvw)\right]}_{\mathrm{Term\ 2}}.
\end{equation}
Most of the time, the log-prior $g$ is relatively simple, e.g., quadratic functions, which means its SDE can be solved with high precision or even with a closed form.
Thus, the exact gradient flow of $\mathrm{Term\ 2}$
in Wasserstein space leads to exponential decay even though discretization error of $\mathrm{Term\ 1}$ will dominate the decrease of the total functional.
Combining this property with the idea of optimizing the two terms alternatively, like composition optimization, the advantage is taken by~\citet{freund2022convergence} in their main algorithm, i.e., Langevin Algorithm with Prior Diffusion (LAPD).
We show a variant in Alg~\ref{alg:lapd}.
Compared with that in~\citet{freund2022convergence}, the main differences lay in two aspects.
First, the order of stages is swapped in our variant, which only leads to the SDE stage at the first iteration being omitted.
Second, the output of Alg~\ref{alg:lapd} is $\tilde{\rvw}_T$ which violates the theoretical analysis in~\citet{freund2022convergence}.

According to the Alg~\ref{alg:lapd}, we introduce some other notations.
Given a random variable $\tilde{\rvw}_0\sim \tilde{p}_0$, we would like to update $\tilde{\rvw}_k\sim \tilde{p}_k$, $t=1,\cdots,T$. 
From a composition optimization perspective, to get an explicit bound on the convergence of the sequence $\{f(\vw_k)\}_{k\in \mathbb{N}_+}$, deduced by the gradient descent type iteration, e.g.,
\begin{equation*}
    \vw_{k+1} = \vw_k - \eta_{k+1}\grad f(\vw_k) + \eta_{k+1}\xi(\vw_k),
\end{equation*}
to the minima $f(\vw_*)$,  one possibility (see~\citet{beck2009A}) is to upper bound function value differences by the distance among variables: \dz{I am not sure whether we need to go with such as detailed derivation in the problem setup section.}
\begin{equation*}
    \begin{aligned}
        &2\eta_{k+1}\left(f(\vw_{k+1})-f(\vw_*)\right)\\
        \le &\left\|\vw_k-\vw_*\right\|^2 - \left\|\vw_{k+1}-\vw_*\right\|^2 + C\eta_{k+1}^2,
    \end{aligned}
\end{equation*}
which highly depends on the convexity of function $f$.
Similarly, the convergence of Eq.~\ref{eq:kl_compos_func} requires
\begin{equation*}
    \begin{aligned}
    & \mathrm{Term\ 1}\rightarrow \mathbb{E}_{\rvw\sim p_*}\left[f(\rvw)\right]\\
    \mathrm{and}\quad &\mathrm{Term\ 2}\rightarrow \mathbb{E}_{\rvw\sim p_*}\left[g(\rvw)+\log p(\rvw)\right].
    \end{aligned}
\end{equation*}
To upper bound the difference between $\mathrm{Term\ 1}$ and its limit with the Wasserstein 2 distance (corresponds to $L_2$ norm in Euclidean space), a crucial assumption is a geodesic convexity of $\mathrm{Term\ 1}$, which can be deduced by the convexity of $f$ in the target distribution $p_*$.
While such a convexity will be violated when $p_*$ only satisfies LSI.

Specifically, we say $p_*$ satisfies LSI with constant $\alpha_*$ if for all smooth
function $\phi\colon \R^d \rightarrow \R$ with $\mathbb{E}_{p_*}[\|\rvw\|^2]\le \infty$,
\begin{equation*}
    \begin{aligned}
    \mathbb{E}_{p_*}\left[\phi^2\ln \phi^2\right]-\mathbb{E}_{p_*}\left[\phi^2\right]\ln \mathbb{E}_{p_*}\left[\phi^2\right]\le \frac{2}{\mu} \mathbb{E}_{p_*}\left[\left\|\nabla \phi\right\|^2\right].
    \end{aligned}
\end{equation*}
By choosing $\phi^2=p/p_*$, we have
\begin{equation*}
        \begin{aligned}        2\alpha_* \mathrm{KL}\left(p\|p_*\right)\le \int p(\vw) \left\|\grad \log\frac{p(\vw)}{p_*(\vw)}\right\|^2 \der\vw\\
        = \int p(\vw) \left\|\frac{\delta \mathrm{KL}\left(p\|p_*\right)}{\delta p}\right\|^2 \der\vw \coloneqq \left\|\mathrm{grad}_p \mathrm{KL}\left(p\|p_*\right) \right\|^2_p,
        \end{aligned}
\end{equation*}
which is just like Polyak-Lojasiewicz (PL) inequality in a geodesic sense~\citep{wibisono2018sampling}.
Similar to the fact that strong convexity can be deduced by PL inequality, LSI applies to a wider class of measures than log-concave distributions and can be checked by Bakry-Emery criterion~\cite{bakry1985diffusions}.
Specifically, bounded perturbation and Lipschitz mapping can preserve the establishment of LSI~\cite{vempala2019rapid}, where log-concavity would be failed.
However, unlike general convergence analysis with PL inequality, the functional Eq.~\ref{eq:kl_compos_func} does not have any property in Wasserstein space which is similar to the smoothness in Euclidean space.
Hence, there is no existing mature solution to extend the analysis of the optimization problem under PL inequality to the sampling problem under LSI inequality except for tracking the dynamics of SDE directly.
On the other hand, we will readily observe that, different from ULA~\citet{vempala2019rapid} described by one single SDE, the two-stage iteration of Alg.~\ref{alg:lapd} makes it challenging to present the dynamic of the particles with one It\^o's SDE.
We defer the solution in the next section.

\begin{algorithm}[t]
    \caption{Langevin Algorithm with Prior Diffusion}
    \label{alg:lapd}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:} Initial distribution $\tilde{p}_0$ on $\R^d$, step size $\{\eta_k\}_{k\in\mathbb{N}}$, target distribution $\exp(-f(x)-g(x))$.
            \STATE Draw $\tilde{\rvw}_0$ from $\tilde{p}_0$.
            \FOR{$k = 1$ to $T$}
                 \STATE{\bfseries Stage1:} Let 
                 \begin{equation*}
                    \rvw_{k} = \tilde{\rvw}_{k-1} - \tilde{\eta}_{k-1}\grad f(\tilde{\rvw}_{k-1}).
                \end{equation*}
                \STATE{\bfseries Stage2:} Sample $\tilde{\rvw}_k$ from $\tilde{\rvw}(\eta_k)$ denoted by the following SDE
                \begin{equation*}
                    \tilde{\rvw}(\eta_k) = \rvw_{k} -\int_0^{\eta_k} \grad g(\tilde{\rvw}(s))\der s + \sqrt{2}\int_0^{\eta_k}\der \mB_t
                \end{equation*}
                 \ENDFOR
                 \STATE {\bfseries Return:}  $\tilde{\rvw}_T$
    \end{algorithmic}
\end{algorithm}

==> 0_contents/030relatedwork_backup.tex <==
\section{Related Work}
\label{sec:related_work}
The non-asymptotic analysis of Langevin algorithm variants has been of interest to the sampling community for a long time, which focuses on the case that the discretization error cannot be ignored (finite step size at time $t$).
%For general Langevin algorithms, most people focus on the non-asymptotic analysis of the convergence rate, which means the step size does not approach to $0$. 
To achieve this result, there are generally two lines to perform the analysis.

The first line is to obtain the contraction of objective functionals by controlling the discretization error between the dynamics of the actual and ideal distribution (or particles).
The actual dynamics of distribution (or particle) usually come from the iteration, and the ideal one comes from the gradient flow of the objective functional.
Specifically, considering Wasserstein 2 distance to the target distribution as the objective functional, ~\citet{dalalyan2017further,dalalyan2019user} first introduced the ideal SDE whose stationary distribution coincides with the target distribution.
Then, they calculate the gap of Wasserstein 2 distances caused by conducting ideal and actual SDE on the current particles.
By controlling this gap with step sizes, the contraction of the objective functional with the actual iteration can be obtained.
Similar techniques are utilized in~\citet{cheng2018convergence,vempala2019rapid}, while they use KL divergence with the target distribution as the objective functional.
Additionally, strong log-concavity of the target distribution is required in~\citet{dalalyan2017further,dalalyan2019user}, and~\citet{cheng2018convergence,vempala2019rapid} replaced the requirements with LSI. However, the continuous ``ideal" dynamics may not always exist for some algorithms, such as the prior diffusion one, so one needs additional construction to perform the analysis. 

The second line is independent of the ideal distribution dynamics converging to the exact target distribution.
It prefers to decompose the objectives into several parts and consider the iteration as a composition optimization algorithm.
For example, ~\citet{durmus2019analysis} decomposes KL divergence into the energy term and the entropy term.
By coupling the iteration of ULA, such two terms are upper bounded with geodesic convexity (or strong convexity), respectively.
A very recent work~\citep{freund2022convergence} expects to find a Langevin algorithm to achieve dimension-independent convergence rate.
The  prior diffusion trick can be considered as re-balancing the coefficients of strong convexity for the energy term and the entropy term in~\citet{durmus2019analysis}. 
It is worth noting that the analysis along this line is similar to the techniques in conventional convex optimization ~\citep{durmus2019analysis} because the geodesic convexity in probability space is extremely similar to the convexity of objectives in  Euclidean space.
However, unlike the first kind of proof, high dependency on geodesic convexity limits its extension to milder assumptions: the analysis under LSI can be hard.

Our analysis can be recognized as an example of the first line where the ``ideal" dynamics are obtained by analytic continuation for each step. Thus, the dimension dependency can be revealed in our work.

\dz{it would be better to categorize these prior works into multiple directions to make this section easier to follow. }

==> 0_contents/040mainresults_backup.tex <==
\section{Theoretical Results}
In this section, we will introduce some assumptions for the posterior sampling problems and demonstrate the  technical comparisons with the early work \citep{freund2022convergence}.
Then, we show the dimension-independent convergence rate of Alg~\ref{alg:lapd} with different step size schedules, e.g., fixing step sizes and varying step sizes, and compare them with previous work.
Finally, we will provide a roadmap for our analysis and the main idea for designing varying step sizes, which helps to understand our theoretical results.
Due to space limitations, we defer details in the Appendix.

\paragraph{Assumptions for all the analysis of this section:}
\begin{enumerate}[label=\textbf{[\Subscript{AS}{\arabic*}]}]
    \item \label{ass:con_post_f} The function $f$ is second derivative, and for any $\vw\in\R^d$, it has
    \begin{equation*}
        \left\|\nabla^2 f(\vw)\right\|\preceq L\mI.
    \end{equation*}
    \item \label{ass:con_post_lsi} The posterior distribution, $p_* \propto \exp(-U)$, satisfies $\alpha_*$ log-Sobolev inequality (LSI), which induces the following relation between KL divergence and Fisher information for all $p$:
    \begin{equation*}
        \mathrm{KL}\left(p\|p_*\right)\le \frac{1}{2\alpha_*}\int p(\vw) \left\|\grad \log\frac{p(\vw)}{p_*(\vw)}\right\|^2 \der\vw.
    \end{equation*}
    \item \label{ass:con_post_f2} Similar to the assumption in Theorem 3 of~\citet{freund2022convergence}, for any $\vw\in\R^d$, we suppose
    \begin{equation*}
        \begin{aligned}
            \vzero\preceq \nabla^2 f(\vw) (\grad^2 f(\vw))^\top \preceq \mH^{\frac{1}{2}}\left(\mH^{\frac{1}{2}}\right)^\top = \mH \preceq L^2\mI,
        \end{aligned}
    \end{equation*}
    where $\mH^{\frac{1}{2}}\succeq \vzero$.
\end{enumerate}
In the following analysis, we will suppose $g(\vw)=(m/2)\left\|\vw\right\|^2$, which is similar to the setting in~\citet{freund2022convergence}.
By choosing the Gaussian prior, \citet{freund2022convergence} actually need the strongly log-concave property for the posterior distribution $p_*$.
 In our analysis, $p_*$ is only required to satisfy LSI, i.e.,~\ref{ass:con_post_lsi}, which is a standard assumption in recent sampling works~\citep{vempala2019rapid,wibisono2019proximal}.
For~\ref{ass:con_post_f2}, due to the general Hessian condition under LSI (may not be positive semi-definite), we require the upper bound for the Hessian square, which is slightly stronger than that (only assuming upper bound of Hessian) in~\citet{freund2022convergence}.
However, similar to~\citet{freund2022convergence},~\ref{ass:con_post_f2} provides the potential for achieving a sharper convergence independent of the dimension number.
%To justify the advantages, \citet{freund2022convergence} has provided several examples in Bayesian machine learning, which can also be handled in our settings due to the excellent property of~\ref{ass:con_post_lsi} and the establishment of~\ref{ass:con_post_f2}.

\paragraph{KL convergence with a fixed step size}
Our main result for Alg~\ref{alg:lapd} can be stated as follows.
\begin{theorem}
    \label{thm:kl_con_fx}
    Assume the posterior $p_*$ satisfies~\ref{ass:con_post_f}-\ref{ass:con_post_f2},and $\alpha_*\le L$ without loss of generality, Alg~\ref{alg:lapd} with step size $\eta_k =\eta \in (0, \hat{\eta}]$ for $k\in\{1,2,\ldots T\}$ and
    \begin{equation*}
        \hat{\eta}\coloneqq \frac{1}{4L^2}\cdot \min\left\{\left(\Tr(\mH^{\frac{1}{2}})+m\right)^{-1}, \frac{8L^2}{3\alpha_*}, \frac{\alpha_*}{2\sqrt{2}}, \frac{\alpha_*L^2\epsilon}{11\mathrm{Tr}(\mH)}\right\}
    \end{equation*}
    satisfies
    \begin{equation*}
        \mathrm{KL}(\tilde{p}_k\|p_*)\le e^{-\alpha_*\hat{\eta} k}\mathrm{KL}(\tilde{p}_0\|p_*) + \frac{32\hat{\eta}}{\alpha_*}\cdot \mathrm{Tr}(\mH).
    \end{equation*}
    In this condition, requiring
    \begin{equation*}
    k\ge \frac{1}{\alpha_* \eta}\log \frac{2\mathrm{KL}(\tilde{p}_0\|p_*)}{\epsilon},
    \end{equation*}
    we have $\mathrm{KL}(\tilde{p}_k\|p_*)\le \epsilon$.
\end{theorem}
This theorem differs from the main results of~\citet{freund2022convergence} from two perspectives.
First, in~\citet{freund2022convergence}, the convergence is about the weighted average of KL divergence at different iterations, which does not correspond to some underline distribution obviously though the weighted average can be achieved with additional steps.
However, Theorem~\ref{thm:kl_con_fx} denotes that dimension-independent convergence can be obtained with only respect to the distribution of $\tilde{\rvw}_T$, and the particle of the last iteration can be output directly.
This property makes the results more clear and practical.
Second, the dimension-free convergence of KL divergence is required decreasing step sizes in~\citet{freund2022convergence}, while Theorem~\ref{thm:kl_con_fx} denotes that fixed step sizes can also achieve a similar result with an additional logarithmic term.

\begin{table*}
    \small
    \centering
    \begin{tabular}{cccc}
    \toprule
     Reference & Assumption & Criterion & Iteration Complexity \\
     \midrule
     \citet{cheng2018convergence} & Convexity of $f$,~\ref{ass:con_post_f} & $\mathrm{KL}\left(\tilde{p}_T\|p_*\right)\le \epsilon$ & $\tilde{\Omega}\left(\frac{L^2}{m^2}\cdot \frac{d}{\epsilon}\right)$\\
     \citet{freund2022convergence} & Convexity of $f$,~\ref{ass:con_post_f},~\ref{ass:con_post_f2} & $\mathrm{KL}\left(\tilde{p}_T\|p_*\right)\le \epsilon$ & $\Omega\left(\frac{L\mathrm{Tr}(\mH^{\frac{1}{2}})}{m^2 \epsilon}+ \frac{U(0)}{\epsilon} \right)$\\
     \midrule
     \citet{vempala2019rapid} & \ref{ass:con_post_f}, \ref{ass:con_post_lsi} & $\mathrm{KL}\left(\tilde{p}_T\|p_*\right)\le \epsilon$ & $\tilde{\Omega}\left(\frac{L^2}{\alpha_*^2}\cdot \frac{d}{\epsilon}\right)$\\
    Theorem~\ref{thm:kl_con_fx} & \ref{ass:con_post_f}, \ref{ass:con_post_lsi}, \ref{ass:con_post_f2} & $\mathrm{KL}\left(\tilde{p}_T\|p_*\right)\le \epsilon$ & $\tilde{\Omega}\left(\frac{\mathrm{Tr}(\mH)}{\alpha_*^2 \epsilon}\right)$\\
    \midrule
    \citet{dalalyan2019user} & Convexity of $f$, \ref{ass:con_post_f} & $W_2^2(\tilde{p}_T, p_*)\le \epsilon$ & $\Omega\left(\frac{L^2}{m^3}\cdot \frac{d}{\epsilon}\right)$\\
    Theorem~\ref{thm:kl_con_vary} & \ref{ass:con_post_f},\ref{ass:con_post_lsi},\ref{ass:con_post_f2}& $W_2^2(\tilde{p}_T, p_*)\le \frac{2}{\alpha_*}\mathrm{KL}\left(\tilde{p}_T\|p_*\right)\le \epsilon$ & $\Omega\left(\frac{\mathrm{Tr}(\mH)}{\alpha_*^3 \epsilon}\right)$\\
     \bottomrule
\end{tabular}
    \caption{Comparison with Previous Results on overdamped Langevin algorithm. Note that the algorithms of the first four lines utilize fixed step sizes, and the last two lines use varying step sizes.}
    \label{tab:comp_old}
\end{table*}

\paragraph{KL convergence with a varying step size}
To get rid of the logarithmic terms in the number of iterations required to achieve the precision level $\epsilon$, we introduce varying step sizes with the inspire of~\citet{dalalyan2019user}.
Hence, we have the following result.
\begin{theorem}
    \label{thm:kl_con_vary}
    Consider Alg~\ref{alg:lapd} with varying step size $\eta_{k+1}$ defined by
    \begin{equation*}
        \eta_{k+1}=\frac{8\hat{\eta}}{9+3(k-K_0)_+\hat{\eta} \alpha_*}
    \end{equation*}
    where $\hat{\eta}$ is denoted as
    \begin{equation*}
        \hat{\eta}\coloneqq \frac{1}{4L^2}\cdot \min\left\{\left(\Tr(\mH^{\frac{1}{2}})+m\right)^{-1}, \frac{8L^2}{3\alpha_*}, \frac{\alpha_*}{2\sqrt{2}}\right\}
    \end{equation*}
    and $K_0$ denotes the smallest non-negative integer satisfying
    \begin{equation*}
        T_0\ge \frac{9}{8\hat{\eta}\alpha_*}\ln\left(\frac{\mathrm{KL}\left(\tilde{p}_0\|p_*\right)\alpha_*}{123\hat{\eta}\mathrm{Tr}(\mH)}\right).
    \end{equation*}
    If the posterior $p_*$ satisfies~\ref{ass:con_post_f}-\ref{ass:con_post_f2} and $\alpha_*\le L$ without loss of generality, for every $k\ge T_0$, we have
    \begin{equation*}
        \mathrm{KL}\left(\tilde{p}_{k}\|p_*\right)\le \frac{2^{10}\cdot \mathrm{Tr}(\mH)}{27L^{1.5}\alpha_*+6\left(k-T_0\right)\alpha^2_*}.
    \end{equation*}
\end{theorem}
The varying step sizes  has two important advantages as compared to the fixed step sizes.
The first is the independence of the target precision level $\epsilon$.
The second advantage is saving the logarithmic terms in Theorem~\ref{thm:kl_con_fx}.
Actually, it suffices
\begin{equation*}
    T = T_0 + \frac{2^9\cdot \mathrm{Tr}(\mH)}{3\epsilon \alpha^2_*}
\end{equation*}
iterations to get $\mathrm{KL}\left(\tilde{p}_T\|p_*\right)\le \epsilon$.
More details of this theorem are provided in Appendix~\ref{appsec:main_results}.
We also provide Table~\ref{tab:comp_old} to show the comparison of assumptions and iteration complexity with several previous work.

\subsection{Proof Sketch}
In this section, we expect to highlight the technical novelties by introducing the roadmap of our analysis.
Due to space limitations, we leave the technical details in Appendix~\ref{appsec:main_results}.

In Section~\ref{sec:problem_setup}, it has demonstrated that for functionals without the geodesic convexity in Wasserstein space, we can hardly upper-bound them by a global metric, e.g., the Wasserstein 2 distance between the current and the target distribution.
From another perspective, different from standard ULA~\citep{dalalyan2017theoretical,vempala2019rapid}, it is not easy to directly find an It\^o's SDE corresponding to the two-stage update of particles.
Therefore, the contraction of KL divergence with Alg~\ref{alg:lapd} remains a mystery in isoperimetry, e.g., log-Sobolev assumption.
To overcome these problems, for each iteration, we utilize a stochastic process $\{\hat{\rvw}_t\}_{t\ge 0}$ deduced by a constructed SDE and required to exist some random variable $\hat{\rvw}_{\eta_k}$ shares the same distribution with the particles after the two-stage update in Alg~\ref{alg:lapd}.
Then, by controlling the difference between such an SDE and the standard gradient flow of KL divergence, we may obtain the discretization error bounded by both $\tilde{\eta}_k$ and $\eta_k$ and prove the contraction of KL divergence in Alg~\ref{alg:lapd}.
Hence, there are two key steps in our analysis:
(1). Find the equivalent It\^o SDE for each two-stage update iteration. (2). Control the error between the constructed It\^o SDE and standard KL divergence flow; see Fig~\ref{fig:M1} for an illustration.

\paragraph{Construction of Equivalent SDE:}
From Alg~\ref{alg:lapd}, the transformation of density function from $\tilde{\rvw}_{k-1}$ to $\tilde{\rvw}_k$ can be considered as a combination of the change of variables (if the step size $\tilde{\eta}_{k-1}$ is small enough) and an Ornstein–Uhlenbeck process (if we suppose $g(\vw)=(m/2)\left\|\vw\right\|^2$).
With the Green's function of OU processes, the probability density of $\tilde{\rvw}_k$ conditioning on $\tilde{\rvw}_{k-1}=\vw_0$ as
\begin{equation*}
     \begin{aligned}
     p(\vw | \vw_0) = \left(\frac{2\pi (1-e^{-2m\eta_k})}{m}\right)^{-d/2} \cdot \exp \left[-\frac{m}{2}\cdot \frac{\left\|\vw-\left(\vw_0 - \tilde{\eta}_{k-1} \grad f(\vw_0)\right) e^{-m\eta_k}\right\|^2}{1-e^{-2m\eta_k}}\right].
     \end{aligned}
\end{equation*}
Besides, various literature, e.g.,~\cite{oksendal2013stochastic} shows that solutions to It\^o SDE are Markov processes.
In a probabilistic sense, it means that all It\^o processes are completely characterized by the transition densities from $\hat{\rvw}_s$ to $\hat{\rvw}_t$, i.e., $p(\vw_t, t|\vw_s, s)$.
Meanwhile, the transition density is also a solution to the Kolmogorov forward equation with a Dirac delta initial density concentrated on $\hat{\rvw}_s$ at time $s$.
Hence, conditioning on $\hat{\rvw}_0 \coloneqq \tilde{\rvw}_{k-1}=\vw_0$, if there is some transition density $p_{\vw_0}(\vw, t|\vw^\prime, t^\prime)$, solving some It\^o SDE, to satisfy 
\begin{equation*}
    p_{\vw_0}(\vw, \eta_k|\vw_0, 0)=p(\vw | \vw_0)
\end{equation*}
for any $\vw\in\R^d$, we consider its corresponding SDE equivalent to the two-stage update in Alg~\ref{alg:lapd}. 
Then, such an equivalent SDE can be constructed by the following lemma.
\begin{lemma}
    \label{lem:con_equivalent_sde}
    Conditioning on $\tilde{\rvw}_{k-1}=\vw_0$, there is a Markov process $\{\hat{\rvw}_t\}_{t\ge 0}$ deduced by the following SDE 
    \begin{equation}
        \label{eq:sde_4.1}
    \der \hat{\rvw}_t = -\left(m\hat{\rvw}_t+\frac{m\tilde{\eta}_{k-1}}{e^{m\eta_k}-1}\grad f(\vw_0)\right)\der t + \sqrt{2}\der \mB_t.
    \end{equation}
Then $\hat{\rvw}_{\eta_k}\sim p_{\vw_0}(\cdot, \eta_k|\vw_0,0)$ shares the same distribution as $\tilde{\rvw}_k$ because 
\begin{equation*}
    \begin{aligned}
        p_{\vw_0}(\vw, \eta_k|\vw_0, 0)=\left(\frac{2\pi (1-e^{-2m\eta_k})}{m}\right)^{-d/2} \cdot \exp \left[-\frac{m}{2}\cdot \frac{\left\|\vw-\left(\vw_0 - \tilde{\eta}_{k-1} \grad f(\vw_0)\right) e^{-m\eta_k}\right\|^2}{1-e^{-2m\eta_k}}\right].
    \end{aligned}
\end{equation*}
\end{lemma}
Roughly speaking, Lemma~\ref{lem:con_equivalent_sde} establishes because the Kolmogorov backward equation of SDE~\ref{eq:sde_4.1}, i.e.,
\begin{equation*}
    \begin{aligned}
        -\frac{\partial p_{\vw_0}(\vw, t| \vw^\prime, t^\prime)}{\partial t^\prime} = \left(-m\vw^\prime - \frac{m\tilde{\eta}_{k-1}}{e^{m\eta_k}-1} \grad f(\vw_0)\right) \cdot \frac{\partial p_{\vw_0}(\vw, t|\vw^\prime, t^\prime)}{\partial \vw^\prime} + 1\cdot \sum_{i=1}^d \frac{\partial^2 p_{\vw_0}(\vw,t | \vw^\prime, t^\prime ,\vw_0)}{\left(\partial \vw_i\right)^2},
    \end{aligned}
\end{equation*}
is solved by the following transition density function
\begin{equation}
    \label{eq:con_trans_kernel}
    \begin{aligned}
        p_{\vw_0}(\vw, t | \vw^\prime, t^\prime) = \left(\frac{2\pi (1-e^{-2m(t-t^\prime)})}{m}\right)^{-d/2} \cdot \exp \left[-\frac{m}{2\left(1-e^{-2m(t-t^\prime)}\right)} \cdot \left\|\vw-\vw^\prime e^{-m(t-t^\prime)} \right.\right.\\
        \left.\left.+ \left(1-e^{-m(t-t^\prime)}\right)\cdot \left(\frac{\tilde{\eta}}{e^{m\eta} -1}\right)\grad f(\vw_0)\right\|^2\right].
    \end{aligned}
\end{equation}
We leave the connection between Kolmogorov equations and transition density in Appendix~\ref{appsec:bke}. 
The more detailed proof of Lemma~\ref{lem:con_equivalent_sde} can be found in Appendix~\ref{sec:implictsde}.

Then, for any suitable probability density function $\tilde{p}_{k-1}$ of $\tilde{\rvw}_{k-1}$, we set
\begin{equation*}
    \hat{p}_t(\vw)\coloneqq \int_{\vw_0} p_{\vw_0}(\vw, t|\vw_0, 0)\cdot \tilde{p}_{k-1}(\vw_0)\der \vw_0,
\end{equation*}
where $p_{\vw_0}$ is the transition density solving SDE.~\ref{eq:sde_4.1}, and
\begin{equation*}
    \begin{aligned}
        \hat{p}_{t|0}(\vw|\vw_0) \coloneqq & p_{\vw_0}(\vw, t|\vw_0, 0), \quad \hat{p}_{0t}(\vw_0, \vw) \coloneqq & \tilde{p}_{k-1}(\vw_0)\cdot p_{\vw_0}(\vw, t|\vw_0, 0)
    \end{aligned}
\end{equation*}
for abbreviation.
Follows from Lemma~\ref{lem:con_equivalent_sde}, we have $\hat{p}_{\eta_k}(\vw)=\tilde{p}_k(\vw)$ for any $\vw\in\R^d$.
It also implies
\begin{equation}
    \label{eq:con_sde_equi}
    \begin{aligned}
        \mathrm{KL}\left(\hat{p}_{\eta_k} \| p^*\right) = &\mathrm{KL}\left(\tilde{p}_{k}\| p^*\right)\quad \mathrm{and}\quad \mathrm{KL}\left(\hat{p}_0 \| p^*\right) = &\mathrm{KL}\left(\tilde{p}_{k-1}\| p^*\right).
    \end{aligned}
\end{equation}
Therefore, the contraction of KL divergence for each iteration of Alg~\ref{alg:lapd} can be obtained by tracking the conditional dynamics shown in SDE.~\ref{eq:sde_4.1}.
\paragraph{Control the variance of particles for each iteration:} Combining Lemma~\ref{lem:con_equivalent_sde} and Eq.~\ref{eq:con_sde_equi}, the equivalent SDE describes a continuously varying KL divergence,
\begin{equation*}
    \small
    \begin{aligned}
        &\mathrm{KL}\left(\tilde{p}_{k}\| p^*\right) - \mathrm{KL}\left(\tilde{p}_{k-1}\| p^*\right)= \mathrm{KL}\left(\hat{p}_{\eta_k} \| p^*\right) - \mathrm{KL}\left(\hat{p}_0 \| p^*\right)\\
        = & \int_0^{\eta_k}\frac{\der \mathrm{KL}\left(\hat{p}_t\|p_*\right)}{\der t} \der t =\int_0^{\eta_k} \int \frac{\partial \hat{p}_t(\vw)}{\partial t}\log \frac{\hat{p}_t(\vw)}{p_*(\vw)}\der \vw \der t,
    \end{aligned}
\end{equation*}
where the dynamics of the distribution $\partial \hat{p}_t/\partial t$ can be obtained by the following fact
\begin{equation*}
    \frac{\partial \hat{p}_t(\vw)}{\partial t}= \int \frac{\partial \hat{p}_{t|0}(\vw|\vw_0)}{\partial t} p_0(\vw_0)\der\vw_0
\end{equation*}
and the Kolmogorov forward equation of SDE.~\ref{eq:sde_4.1}. 
By choosing step sizes, i.e., $\tilde{\eta}_{k-1}$ and $\eta_k$, appropriately, the dynamic of KL divergence has the following bound
\begin{equation*}
    \begin{aligned}
        \frac{\der \mathrm{KL}\left(\hat{p}_t\|p_*\right)}{\der t} \le -\frac{3\alpha_*}{2}\cdot\mathrm{KL}(\hat{p}_t\|p_*)
        + \underbrace{\int \hat{p}_{0t}\left(\vw_0, \vw\right)\left\|\grad f(\vw_0)-\grad f(\vw)\right\|^2 \der (\vw_0, \vw)}_{\mathrm{discretization\ error}}
    \end{aligned}
\end{equation*}
when the target distribution satisfies~\ref{ass:con_post_lsi}.
Actually, the discretization error is from the difference between SDE~\ref{eq:sde_4.1} and the standard Langevin dynamics
\begin{equation*}
    \der \hat{\rvw}_t = -\left(m\hat{\rvw}_t+\grad f(\hat{\rvw}_t)\right)\der t + \sqrt{2}\der \mB_t.
\end{equation*}
To control the error, we introduce the mean of particles along SDE~\ref{eq:sde_4.1} at time $t$ given $\vw_0$, i.e.,
\begin{equation*}
    \overline{\vw}(t, \vw_0)=e^{-mt}\vw_0 - \frac{1-e^{-mt}}{m} \grad f(\vw_0),
\end{equation*}
which can be obtained by the transition density Eq.~\ref{eq:con_trans_kernel}. 
The discretization error can be divided into two parts, relating to the bias of the particles' mean, i.e.,
\begin{equation}
    \label{ineq:con_meanerr}
    \int \hat{p}_0(\vw_0) \left\|\grad f(\overline{\vw}(t,\vw_0)) -\grad f(\vw_0)\right\|^2 \der\vw_0,
\end{equation}
and their variance, i.e.,
\begin{equation}
    \small
    \label{ineq:con_varerr}
    \int \hat{p}_0(\vw_0) \int \hat{p}_{t|0}(\vw|\vw_0)\left\|\grad f(\vw)-\grad f(\overline{\vw}(t,\vw_0))\right\|^2\der \vw \der\vw_0,
\end{equation}
at time $t$ along SDE~\ref{eq:sde_4.1}.
Actually, with the definition of particles' mean and smooth properties (\ref{ass:con_post_f} and~\ref{ass:con_post_f2}), Eq.~\ref{ineq:con_meanerr} can be controlled by $\mathcal{O}(\eta_k^2)$.
While due to the Gaussian-type distribution $\hat{p}_{t|0}$, Eq.~\ref{ineq:con_varerr} only has the following upper bound
\begin{equation*}
     \frac{1-e^{-2mt}}{m}\cdot\mathrm{Tr}(\mH) = \mathcal{O}(\eta_k).
\end{equation*}
Due to a small enough discretization error required by the convergence of sampling algorithms, we know such an error is dominated by the error relating to particles' variance along the SDE from the previous upper bounds. However, introducing the variance of particles is necessary. Otherwise, we may find other ways to control the entropy term in KL divergence. 
Another result to note is that the coefficient of the leading term of the error is not related to the number of dimensions $d$ but to some second derivative properties of function $f$, i.e., $\mathrm{Tr}(\mH)$.
It means that even though there exists the dependency of $d$ in error relating to the bias of the particles' mean, it will also diminish with the decrease of the tolerance of KL divergence error.
Therefore, the contraction of KL divergence with Alg~\ref{alg:lapd} is given as the following lemma.
\begin{lemma}
    \label{lem:con_kl_contraction}
    Suppose the target distribution $p_*$ satisfies~\ref{ass:con_post_f}-~\ref{ass:con_post_f2}, if we set
    \begin{equation*}
        \left(m\tilde{\eta}_{k-1}\right)/\left(e^{m\eta_k}-1\right)=1
    \end{equation*}
    and
    \begin{equation}
        \label{ineq:step0_upb}
        0< \eta_k\le \frac{1}{4L^2}\cdot \min\left\{\left(\Tr(\mH^{\frac{1}{2}})+m\right)^{-1}, \frac{8L^2}{3\alpha_*}, \frac{\alpha_*}{2\sqrt{2}}\right\},
    \end{equation}
    then along each iteration of Alg~\ref{alg:lapd}, it has
    \begin{equation*}
        \mathrm{KL}(\tilde{p}_{k}\|p_*)\le e^{-\alpha_*\eta_k}\mathrm{KL}(\tilde{p}_{k-1}\|p_*) + 16\eta_k^2\mathrm{Tr}(\mH).
    \end{equation*}
\end{lemma}
\begin{figure}
\input{0_figs/proof_explain.tex}
\caption{An illustration for the proof of Lemma~\ref{lem:con_kl_contraction}. In each iteration, we compare the evolution of
(a) the continuous-time KL divergence flow for time $\eta_k$, and (b) the constructed SDE equivalent to two-stage update at time $\eta_k$.} \label{fig:M1}
\end{figure}
\paragraph{Design the schedule of varying step size:} In this part, we will introduce some intuitions about the design of varying step size in Theorem~\ref{thm:kl_con_vary}.
Starting from the contraction of KL divergence for each iteration, i.e., Lemma~\ref{lem:con_kl_contraction}, we have
\begin{equation*}
    \mathrm{KL}(\tilde{p}_{k}\|p_*)\le e^{-\alpha_*\eta_k}\mathrm{KL}(\tilde{p}_{k-1}\|p_*) + 24\eta_k^2\mathrm{Tr}(\mH)
\end{equation*}
under some constraints of $\eta_k$, i.e.,~Eq.~\ref{ineq:step0_upb}.
Without loss of generality, we suppose $\alpha_*\le L$ and the contraction of KL divergence can be relaxed as
\begin{equation*}
    \mathrm{KL}(\tilde{p}_{k}\|p_*)\le \left(1-\frac{3}{4}\alpha_* \eta_k\right)\mathrm{KL}(\tilde{p}_{k-1}\|p_*) + 24\eta_k^2\mathrm{Tr}(\mH).
\end{equation*}
We use the auxiliary sequence $\{B_k\}_{k\ge 0}$ and expect it upper bounds the KL divergence at each iteration, i.e.,
\begin{equation}
    \label{ineq:kl_upb_varying}
    B_k \ge \frac{3 \alpha_*^2}{2^9\cdot \mathrm{Tr}(\mH)}\mathrm{KL}\left(\tilde{p}_k\|p_*\right).
\end{equation}
Such an inequality can be established by setting the suitable initialization (Eq.~\ref{ineq:kl_upb_varying} established at $k=T_0$) and the
proper contraction of $B_k$ which corresponds 
 to that of the upper bound of KL divergence when $k\ge T_0$, i.e.,
\begin{equation*}
    \begin{aligned}
        B_{k+1} = \left(1-\frac{3}{4}\alpha_* \eta_{k+1}\right)B_k + \frac{9}{64}\alpha_*^2\eta_{k+1}^2.
    \end{aligned}
\end{equation*} 
Minimizing the RHS w.r.t. $\eta_{k+1}$, we can build the connection between the auxiliary sequence and the  step size, 
\begin{equation}
    \label{eq:connection_B_eta}
    -\frac{3}{4}\alpha_* B_k + \frac{9}{32}\alpha_*^2\eta_{k+1} = 0 \Leftrightarrow B_k = \frac{3}{8}. \alpha_* \eta_{k+1}.
\end{equation}
In this condition, $B_k$ satisfies the following  inequality
\begin{equation*}
    \begin{aligned}
        B_k \le & B_k\left(1-2B_k\right)+B_k^2 = B_k\left(1-B_k\right)\le \frac{B_k}{1+B_k},
    \end{aligned}
\end{equation*}
where the last inequality follows from the positivity of KL divergence.
Besides, the function $x/(1+x)$ is increasing on $(0,+\infty)$, it means we have
$$
    B_{k+1}\le \frac{B_k}{1+B_k}\le \frac{\frac{B_{k-1}}{1+B_{k-1}}}{1+\frac{B_{k-1}}{1+B_{k-1}}} = \frac{B_{k-1}}{1+2B_{k-1}}.
$$
Recursively applying such an inequality, we have
$$
    B_{k+1} \le \frac{B_{T_0}}{1+(k+1-T_0)B_{T_0}},
$$
for any $T_0$.

Then, we can construct the auxiliary sequence through its connection with step sizes, i.e., Eq.~\ref{eq:connection_B_eta}. 
First, considering the constraints of $\eta_k$, we may require $B_{T_0}$ to be small enough.
Therefore, we can choose 
\begin{equation*}
    \eta_{T_0+1} =\frac{8}{3\alpha_*}\cdot B_{T_0} \coloneqq \frac{8\hat{\eta}}{9} = \frac{8\hat{\eta}}{9+3\hat{\eta}\alpha_*\left(T_0-T_0\right)}\le \hat{\eta}
\end{equation*}
and construct the general formula of $\eta_{k+1}$ as
\begin{equation*}
    \eta_{k+1} \coloneqq \frac{8}{3\alpha_*}\cdot \frac{\alpha_*\hat{\eta}}{3+\left(k-T_0\right)\alpha_* \hat{\eta}}.
\end{equation*}
This construction allows the following recursive inequality
\begin{equation*}
    B_{k} = \frac{3\alpha_*}{8}\eta_{k+1} = \frac{\alpha_*\hat{\eta}}{3+\left(k-T_0\right)\alpha_* \hat{\eta}} = \frac{B_{T_0}}{1+(k-T_0)B_{T_0}}.
\end{equation*}
Hence, the auxiliary sequence and varying step sizes are constructed.
The detailed proof is provided in Appendix~\ref{appsec:main_results}.



\paragraph{Control the variance of particles for each iteration.} Combining Lemma~\ref{lem:con_equivalent_sde} and Eq.~\ref{eq:con_sde_equi}, the equivalent SDE describes a continuously varying KL divergence,
\begin{equation*}
    \small
    \begin{aligned}
        &\mathrm{KL}\left(\tilde{p}_{k}\| p^*\right) - \mathrm{KL}\left(\tilde{p}_{k-1}\| p^*\right)= \mathrm{KL}\left(\hat{p}_{\eta_k} \| p^*\right) - \mathrm{KL}\left(\hat{p}_0 \| p^*\right)\\
        = & \int_0^{\eta_k}\frac{\der \mathrm{KL}\left(\hat{p}_t\|p_*\right)}{\der t} \der t =\int_0^{\eta_k} \int \frac{\partial \hat{p}_t(\vw)}{\partial t}\log \frac{\hat{p}_t(\vw)}{p_*(\vw)}\der \vw \der t,
    \end{aligned}
\end{equation*}
where the dynamics of the distribution $\partial \hat{p}_t/\partial t$ can be obtained by the following fact
\begin{equation*}
    \frac{\partial \hat{p}_t(\vw)}{\partial t}= \int \frac{\partial \hat{p}_{t|0}(\vw|\vw_0)}{\partial t} p_0(\vw_0)\der\vw_0
\end{equation*}
and the Kolmogorov forward equation of SDE.~\ref{eq:sde_4.1}. 
By choosing step sizes, i.e., $\tilde{\eta}_{k-1}$ and $\eta_k$, appropriately, the dynamic of KL divergence has the following bound
\begin{equation*}
    \begin{aligned}
        \frac{\der \mathrm{KL}\left(\hat{p}_t\|p_*\right)}{\der t} \le -\frac{3\alpha_*}{2}\cdot\mathrm{KL}(\hat{p}_t\|p_*)
        + \underbrace{\int \hat{p}_{0t}\left(\vw_0, \vw\right)\left\|\grad f(\vw_0)-\grad f(\vw)\right\|^2 \der (\vw_0, \vw)}_{\mathrm{discretization\ error}}
    \end{aligned}
\end{equation*}
when the target distribution satisfies~\ref{ass:con_post_lsi}.
Actually, the discretization error is from the difference between SDE~\ref{eq:sde_4.1} and the standard Langevin dynamics
\begin{equation*}
    \der \hat{\rvw}_t = -\left(m\hat{\rvw}_t+\grad f(\hat{\rvw}_t)\right)\der t + \sqrt{2}\der \mB_t.
\end{equation*}
To control the error, we introduce the mean of particles along SDE~\ref{eq:sde_4.1} at time $t$ given $\vw_0$, i.e.,
\begin{equation*}
    \overline{\vw}(t, \vw_0)=e^{-mt}\vw_0 - \frac{1-e^{-mt}}{m} \grad f(\vw_0),
\end{equation*}
The discretization error can be divided into two parts, relating to the bias of the particles' mean, i.e.,
\begin{equation}
    \label{ineq:con_meanerr}
    \int \hat{p}_0(\vw_0) \left\|\grad f(\overline{\vw}(t,\vw_0)) -\grad f(\vw_0)\right\|^2 \der\vw_0,
\end{equation}
and their variance, i.e.,
\begin{equation}
    \small
    \label{ineq:con_varerr}
    \int \hat{p}_0(\vw_0) \int \hat{p}_{t|0}(\vw|\vw_0)\left\|\grad f(\vw)-\grad f(\overline{\vw}(t,\vw_0))\right\|^2\der \vw \der\vw_0,
\end{equation}
at time $t$ along SDE~\ref{eq:sde_4.1}.
Actually, with the definition of particles' mean and smooth properties (\ref{ass:con_post_f} and~\ref{ass:con_post_f2}), Eq.~\ref{ineq:con_meanerr} can be controlled by $\mathcal{O}(\eta_k^2)$.
While due to the Gaussian-type distribution $\hat{p}_{t|0}$, Eq.~\ref{ineq:con_varerr} only has the following upper bound
\begin{equation*}
     \frac{1-e^{-2mt}}{m}\cdot\mathrm{Tr}(\mH) = \mathcal{O}(\eta_k).
\end{equation*}
Due to a small enough discretization error required by the convergence of sampling algorithms, we know such an error is dominated by the error relating to particles' variance along the SDE from the previous upper bounds. However, introducing the variance of particles is necessary. Otherwise, we may find other ways to control the entropy term in KL divergence. 
Another result to note is that the coefficient of the leading term of the error is not related to the number of dimensions $d$ but to some second derivative properties of function $f$, i.e., $\mathrm{Tr}(\mH)$.
It means that even though there exists the dependency of $d$ in error relating to the bias of the particles' mean, it will also diminish with the decrease of the tolerance of KL divergence error.
Therefore, the contraction of KL divergence with Alg~\ref{alg:lapd} is given as the following lemma.

==> 0_contents/050conclusion_backup.tex <==
\section{Discussion}
\label{sec:diss}
This section mainly compares our analysis  with the standard Unadjusted Langevin Algorithm (ULA) and demonstrates the advantages of Alg~\ref{alg:lapd}.
Specifically, similar to~\citet{freund2022convergence}, we show the convergence rate on ridge separable $f$ and quadratic $g$ as an example.

For the previous analysis of ULA, e.g.,~\citet{vempala2019rapid}, the convergence rate can also be improved by decomposing the discretization error into the particles' mean relating part, e.g., Eq.~\ref{ineq:con_meanerr} and the variance relating part, e.g., Eq.~\ref{ineq:con_varerr}.
In this condition, the convergence rate dominated by the particles' variance relating error (the leading term) can be upper bounded by the trace of Hessian of $U$ rather than the dimension number $d$, which sharpens the existing analysis.
Even in this condition, the analysis of ULA can only be considered a special case of our results when the coefficients of $g$, i.e., $m$, approximate $0$.
Due to the arbitrary choice of $m$, Alg~\ref{alg:lapd}  essentially provides the possibility for translation transformation of the negative log target density spectrum without additional discretization error.
It is actually presented as that the convergence result of Alg~\ref{alg:lapd} is about the trace of Hessian of $f$ rather than $U$.
Therefore, the theoretical result of Alg~\ref{alg:lapd} will be strictly better than that of ULA.
Specifically, if we know the Hessian of $U$ at each point $\vw$, supposing the eigenvalues of $\grad^2 U(\vw)$ is $\{\sigma_i\}_{i\ge 1}^d$
we can even calculate the optimal $m$ w.r.t. $\vw$ by the following equation
\begin{equation*}
    m_* = \arg\min_{c}\quad \sum_{i=1}^d (\sigma_i-c)^2 = \frac{1}{d}\sum_{i=1}^d \sigma_i,
\end{equation*}
though we use a uniform $m$ in Alg~\ref{alg:lapd} for all $\vw\in\R$.
With this benefit, a natural question is when this trick will significantly improve the convergence rate.
First, when the eigenvalues of negative log-likelihood, i.e., $\grad^2 f(\vw)$, decrease sharply, e.g., following from power law, the translate transformation will directly work on the Gaussian prior.
Another practical example is provided in the following to demonstrate the efficiency of LAPD. 
We may consider $p_*$ as a simple Gaussian mixture density function presented as follows $p_*(\vw) \propto \frac{1}{n}\sum_{i=1}^n \exp\left(-\frac{1}{2}\left\|\vw-\boldsymbol{\mu}_i\right\|^2\right)$, which means
\begin{equation*}
    U_*(\vw)= -\ln\left[\frac{1}{n}\sum_{i=1}^n e^{\boldsymbol{\mu}_i^\top \vw - \frac{1}{2}\left\|\boldsymbol{\mu}_i\right\|^2}\right]+\frac{1}{2}\left\|\vw\right\|^2 \coloneqq f_*(\vw)+g_*(\vw).
\end{equation*}
We should note that $p_*$ is not strongly log-concave but satisfies log-Sobolev inequality~\cite{chen2021dimension}.
Then, we consider the properties of $f_*$ and have
\begin{equation*}
        \grad f_*(\vw) = -\left(\sum_{i=1}^n \exp(\boldsymbol{\mu}_i^\top \vw - \frac{1}{2}\|\boldsymbol{\mu}_i\|^2)\right)^{-1}\cdot \sum_{i=1}^n \exp(\boldsymbol{\mu}_i^\top \vw - \frac{1}{2} \|\boldsymbol{\mu}_i\|^2)\boldsymbol{\mu}_i.
\end{equation*}
To simplify the notation, if we define $v_i=\exp(\boldsymbol{\mu}_i^\top \vw - \frac{1}{2} \|\boldsymbol{\mu}_i\|^2)\in\R_+$, then we have

\begin{equation*}
    \begin{aligned}
        \grad^2 f_*(\vw) = &\left(\sum_{i=1}^n v_i\right)^{-2}\cdot \left(\sum_{i=1}^n v_i\boldsymbol{\mu}_i \sum_{j=1}^n v_j\boldsymbol{\mu}_j^\top - \sum_{i=1}^n v_i\boldsymbol{\mu}_i\boldsymbol{\mu}_i^\top \sum_{j=1}^n v_j\right)\\
        = & -\frac{1}{2}\left(\sum_{i=1}^n v_i\right)^{-2}\cdot\sum_{1\le i\le j\le n} v_iv_j\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)^\top.
    \end{aligned}
\end{equation*}
We may set $\mH^{1/2} = \sum_{1\le i\le j\le n}\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)^\top$, because $0 \preceq -\grad^2 f_* \preceq \frac{1}{2}\mH^{1/2}$. Hence, it has
\begin{equation*}
    \begin{aligned}
    \mathrm{Tr}(\mH) \le \mathrm{Tr}(\mH^{1/2})^2 = \Tr\left(\sum_{1\le i\le j\le n}\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)^\top\right)^2 \le 16n^4R_{\mu}^4,
    \end{aligned}
\end{equation*}
where the means of the Gaussian mixture satisfy $\|\boldsymbol{\mu}_i\|\le R_{\mu}$.
In this case, the convergence of LAPD is only dependent on the mixture components $n$ and the radius of means $R_{\mu}$, rather than the dimension number $d$.


\begin{example}
\end{example}

\section{Conclusion}
In this paper, we analyze the complexity of (unadjusted) Langevin algorithm with prior diffusion in KL divergence. By tracking the dynamics of the proposed algorithm and discretization errors, we obtain that the convergence of the algorithm can be dimension independent with both fixed and varying step sizes under log-Sobolev inequality. 

Then, we consider the properties of $f_*$ and have
\begin{equation*}
        \grad f_*(\vw) = -\left(\sum_{i=1}^n \exp(\boldsymbol{\mu}_i^\top \vw - \frac{1}{2}\|\boldsymbol{\mu}_i\|^2)\right)^{-1}\cdot \sum_{i=1}^n \exp(\boldsymbol{\mu}_i^\top \vw - \frac{1}{2} \|\boldsymbol{\mu}_i\|^2)\boldsymbol{\mu}_i.
\end{equation*}
To simplify the notation, if we define $v_i=\exp(\boldsymbol{\mu}_i^\top \vw - \frac{1}{2} \|\boldsymbol{\mu}_i\|^2)\in\R_+$, then we have

\begin{equation*}
    \begin{aligned}
        \grad^2 f_*(\vw) = &\left(\sum_{i=1}^n v_i\right)^{-2}\cdot \left(\sum_{i=1}^n v_i\boldsymbol{\mu}_i \sum_{j=1}^n v_j\boldsymbol{\mu}_j^\top - \sum_{i=1}^n v_i\boldsymbol{\mu}_i\boldsymbol{\mu}_i^\top \sum_{j=1}^n v_j\right)\\
        = & -\frac{1}{2}\left(\sum_{i=1}^n v_i\right)^{-2}\cdot\sum_{1\le i\le j\le n} v_iv_j\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)\left(\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\right)^\top.
    \end{aligned}
\end{equation*}

==> 0_contents/abstract_backup.tex <==
Langevin algorithms are usually recognized as first-order optimization methods in probability space, which take the gradient flow of the Kullback-Leibler (KL) divergence. Notably, unlike the gradient-based methods in conventional optimization, the iteration complexity of most Langevin algorithms depends on the dimension, {which is unacceptable for overparameterized models.} 
However, \cite{freund2022convergence} suggest that
the modified Langevin algorithm with prior diffusion is able to converge dimension independently for strongly log-concave target distributions, which encounters the results in conventional optimization. 
Nonetheless, it remains open whether such property establishes for more general cases.
In this paper, we investigate the prior diffusion trick for target distributions satisfying log-Sobolev inequality (LSI), which covers strongly log-concave and even some non-log-concave target distributions.
Under this more general assumption, we prove the modified Langevin algorithm can also obtain the dimension-independent convergence of KL divergence with different step size schedules.
By comparing our analysis with the previous, we demonstrate the benefits of prior diffusion from a theoretical perspective.
In summary, our analysis provides new insights into the dimension dependency of Langevin algorithms under LSI.

\dz{I am not sure whether using nearly half of the paragraph to motivate this work is a good idea. I guess we do not need to mention optimization. Perhaps we can go with (1) improving the dimension dependency in high-dimensional sampling problem is important; (2) There is a possible solution, but can only work for strongly log-concave distribution; (3) we extend to more general cases, LSI and proving a nearly dimension-independent bound; (4) mentioning the key step is to XXX.}
%We extend this result for the target distribution log-Sobolev inequality


 %in terms of Kullback–Leibler (KL) divergence. 
%With log-Sobolev inequality, our algorithm 
  
 % By introducing a reweighted kernel, we provide a novel analysis to obtain the convergence rate of SVGD in the population limit without Stein log-Sobolev inequality.
